Kmt-2016-blg-1397b: Kmtnet-only discovery of a microlens giant planet

We report the discovery of a giant planet in the KMT-2016-BLG-1397 microlensing event, which was found by The Korea Microlensing Telescope Network (KMTNet) alone. The time scale of this event is t_E = 40.0 +- 0.5 days and the mass ratio between the lens star and its companion is q = 0.016 +- 0.002. The planetary perturbation in the light curve is a smooth bump, resulting in the classical binary-lens/binary-source (2L1S/1L2S) degeneracy. We measure the V - I color of the (putative) two sources in the 1L2S model, and then effectively rule out the binary source solution. The finite-source effect is marginally detected. Combined with the limits on the blend flux and the probability distribution of the source size normalized by the Einstein radius rho, a Bayesian analysis yields the lens mass M_L = 0.45+0.33-0.28 M_sun, at distance of D_L = 6.60+1.10-1.30 kpc. Thus the companion is a super-Jupiter of a mass m_p = 7.0+5.2-4.3 M_J , at a projected separation r = 5.1+1.5-1.7 AU, indicating that the planet is well beyond the snow line of the host star.

==> lens.tex <==
\subsection{Color-Magnitude Diagram}\label{cmd}
To further constrain the lens properties, we estimate the angular radius $\theta_*$ of the source by placing the source on a color-magnitude diagram (CMD) \citep{Yoo2004}. We construct the CMD by stars within a $120^{\prime\prime}$ square centered on the source position using KMTC data. We estimate the red clump to be $(V-I, I)_{\rm cl} = (2.41\pm0.02, 13.91\pm0.06)$ and find that the source is $\Delta(V - I) = -0.44\pm0.03$ bluer and $\Delta I = 2.23\pm0.08$ fainter than the red clump. From \cite{Bensby2013,Nataf2013}, we find that the intrinsic color and de-reddened brightness of the red clump are $(V-I, I)_{\rm cl,0} = (1.06, 14.27)$. Thus, the intrinsic color and de-reddened magnitude of the source are $(V-I, I)_{\rm S,0} = (0.62\pm0.03, 16.50\pm0.08)$. We then employ the color/surface-brightness relation in \cite{Adams2018}, and finally find 
\begin{equation}\label{angular}
    \an =  1.50 \pm 0.06~\mu {\rm as}.
\end{equation}

For the binary-lens models, we obtain a $3\sigma$ upper limit $\rho<0.046$. This allows us to set a lower limit on the angular Einstein radius $\theta_{\rm E}$,
\begin{equation}
    \thetae > \frac{\theta_*}{\rho_{\rm upper}} = 0.033~\text{mas}.
\end{equation}

We can also estimate the effective temperature $T_{\rm eff} = 6000~$K of the source by using the color-temperature relation in \cite{Houdashelt2000}. Using ATLAS models and assuming a metallicity of [M/H] = 0.0, a microturbulence parameter of 1 km/s and a surface gravity of $\log g$ = 4.0, we obtain the linear limb-darkening coefficients $u_I = 0.4679$ for $I$ band,  $u_V = 0.6252$ for $V$ band \citep{Claret2011}. This, when combined with the transformation formula in \cite{Fields2013}, yields the corresponding limb-darkening coefficients $\Gamma_{I} = 0.3696$, $\Gamma_{V} = 0.5625$. 

\subsection{Bayesian analysis}\label{Bayesian}
For a lensing object, the total mass $M_{\rm L}$ and distance $D_{L}$ is related to observables by
\begin{equation}
    M_{\rm L} = \frac{\thetae}{{\kappa}\pie};~
    D_{\rm L} = \frac{\mathrm{au}}{\pie\thetae + \pi_{\rm S}},
    \label{eq:mass}
\end{equation}
where $\kappa \equiv 4G/(c^2\mathrm{au}) = 8.144$ mas$/M_{\odot}$ is a constant, $\thetae$ is the angular Einstein radius, $\pie$ is the microlensing parallax~\citep[e.g.,][]{Gould2000} and $\pi_{\rm S} = \mathrm{au}/D_{\rm S}$ is the source parallax \citep{Gouldpies1992,Gouldpies2004}. For KMT-2016-BLG-1397, neither $\thetae$ nor $\pie$ is unambiguously measured. However, combining the timescale $t_{\rm E}$, the limits of blend flux and the probability distribution of $\rho$, we can use Bayesian analysis to estimate the mass and distance of the lens system.

We applied the Galactic model and Bayesian model described in \cite{Zhu2017spitzer} to randomly draw lensing events. We weight all events by exp($-\Delta\chi^2(\rho)/2$), where $\Delta\chi^2(\rho)$ represents the $\chi^2$ difference relative to the minimum $\chi^2$ for the lower envelope of the ($\chi^2$ vs.~$\rho$) diagram derived from the MCMC. In addition, the blend flux is $I_{\rm b,inst} = 17.92 \pm 0.15$, To be conservative, we set an upper limit of the blend flux to be $I_{\rm b,limit} = 17.47~(3\sigma)$. We adopt the mass-luminosity relation \citep{OB171130},
\begin{equation}
    M_I = 4.4 - 8.5 \log{\frac{M}{M_{\odot}}},
\end{equation}
where $M_I$ is the absolute magnitude in $I$-band. We reject trial events for which the lens distance obeys 
\begin{equation}
    M_I + 5 \log{\frac{D_{\rm L}}{10 {\rm pc}}} < I_{\rm b,limit} - \Delta I_{\rm cl},
\end{equation}
where $\Delta I_{\rm cl} = I_{\rm cl} - I_{\rm cl,0} = -0.36$. The resulting posterior distributions of the lens mass $M_{\rm L}$, distance $D_{\rm L}$, lens-source relative proper motion $\mu$ and the projected separation $r_\perp$ of the planet are shown in Figure \ref{fig:baye}. We find that the lens mass is $M_{\rm L} = 0.45_{-0.28}^{+0.33}~M_\odot$.  The uncertainties are the $68\%$ probability range about the median of the probability distribution, which we take as the most likely value. Thus the planet mass is $M_{\rm planet} = 7.0_{-4.3}^{+5.2}~M_{J}$. The lens distance is $D_{\rm L} = 6.60_{-1.30}^{+1.10}$~kpc, and the planet is at a projected separation $r_\perp = 5.1_{-1.7}^{+1.5}$~AU from the host star, indicating that the planet is well beyond the snow line of the host star (assuming a relation $r_{\rm SL} = 2.7(M/M_{\odot})$~{\rm AU}, \citealt{snowline}).

